Understanding the Effects of Second-Order Approximations in Natural Policy Gradient Reinforcement Learning

Natural policy gradient methods are popular reinforcement learning methods that improve the stability of policy gradient methods by utilizing second-order approximations to precondition the gradient with the inverse of the Fisher-information matrix. However, to the best of the authors' knowledge, there has not been a study that has investigated the effects of different second-order approximations in a comprehensive and systematic manner. To address this, five different second-order approximations were studied and compared across multiple key metrics including performance, stability, sample efficiency, and computation time. Furthermore, hyperparameters which aren't typically acknowledged in the literature are studied including the effect of different batch sizes and optimizing the critic network with the natural gradient. Experimental results show that on average, improved second-order approximations achieve the best performance and that using properly tuned hyperparameters can lead to large improvements in performance and sample efficiency ranging up to +181%. We also make the code in this study available at https://github.com/gebob19/natural-policy-gradient-reinforcement-learning.

==> test.tex <==
\hypertarget{title-understanding-the-effects-of-second-order-approximations-in-natural-policy-gradient-reinforcement-learning}{%
\section{Title: Understanding the Effects of Second-Order Approximations
in Natural Policy Gradient Reinforcement
Learning}\label{title-understanding-the-effects-of-second-order-approximations-in-natural-policy-gradient-reinforcement-learning}}

\hypertarget{introduction}{%
\section{Introduction}\label{introduction}}

The policy gradient method {[}@sutton2000policy{]} is a popular
optimization method for reinforcement learning problems however, it
suffers from unstable training due to high-variance gradient estimates
{[}@mohamed2020monte{]}. A promising solution is to leverage natural
policy gradient methods, which preconditions the gradient with the
inverse of the Fisher-information matrix {[}@Amari1998{]} to restrict
how much the model's predictions can change between training iterations.

For neural networks, which can have tens of millions of parameters,
directly computing the inverse of the Fisher-information matrix is
intractable since the Fisher-information matrix is an
\(n_\theta \times n_\theta\) matrix, where \(n_\theta\) is the number of
parameters in the model. This led to the research community developing
new approximations for the inverse of the Fisher-information matrix
which led to having to choose the most appropriate approximation method.
Furthermore, to generate effective performance, setting the batch size
and how to optimize the critic network are also important details. To
the best of the authors' knowledge, there has not been a study that has
holistically investigated strategies for choosing these details to
achieve high performance with natural policy gradient methods in a
comprehensive and systematic manner.

In this paper, we study the effects of five different second-order
approximations: Hessian-free optimization (HF), diagonal approximations
(Diagonal), Kronecker-factored approximate curvature (KFAC),
Eigenvalue-corrected Kronecker factorization approximate curvature
(EKFAC), and Time-efficient natural gradient descent (TENGraD).

Across these approximations, we investigate training strategies which
arent typically given importance in policy gradient research including,
the effect of using different batch sizes and the effect of using
different optimization methods on the critic network.

We study these approximations and training strategies across multiple
reinforcement learning environments and record statistics on
performance, training stability, sample efficiency, and computation
time.

\hypertarget{background}{%
\section{Background}\label{background}}

In this section, we first introduce notation used throughout the paper
and then give a brief overview of the policy gradient method, the
natural policy gradient method, and the five different second-order
approximations which can be used to implement the natural policy
gradient method.

\hypertarget{notation}{%
\subsection{Notation}\label{notation}}

We consider an infinite-horizon discounted Markov decision process,
defined by the tuple (\(\mathcal{S}\), \(\mathcal{A}\), \(p\), \(r\),
\(\gamma\)) which defines the state distribution \(\mathcal{S}\), action
distribution \(\mathcal{A}\), state transition function \(p\), reward
function \(r\), and discount factor \(\gamma\). Specifically, at time
\(t\), an agent is in a state \(s_t \in \mathcal{S}\) and samples an
action \(a_t \in \mathcal{A}\) from its policy, \(\pi (a_t | s_t)\). The
environment then produces a reward \(r(a_t, s_t)\) and a new state
\(s_{t+1} \in \mathcal{S}\) according to the transition probability
function \(p(s_{t+1} | a_t, s_t)\). Repeating this process \(n\) times
produces a trajectory, \(\tau\), of length \(n\).

\hypertarget{policy-gradient-methods}{%
\subsection{Policy Gradient Methods}\label{policy-gradient-methods}}

The policy gradient method {[}@sutton2000policy{]} parameterizes its
policy with parameters \(\theta\) and aims to minimize the negative
expected reward of its trajectories:

\[\underset{\theta}{\mathop{\mathrm{argmin}}} \, L(\theta) = \underset{\theta}{\mathop{\mathrm{argmin}}} \, - \mathbb{E}_{\tau \sim \pi(\tau | \theta)} [r(\tau) \,|\, \pi(\cdot | \theta)]
    ****\]

where for each time step \(t\) in the trajectory \(\tau\):
\(r(\tau)_t = \sum_{i=0}^\infty \gamma^i r(a_{t+i}, s_{t+i})\) is the
discounted cumulative reward after taking action \(a_t\) in state
\(s_t\) and \(\pi(\cdot | \theta)_t = \pi (a_t | s_t, \theta)\) is the
policy's probability of taking action \(a_t\). In general, to optimize
\protect\hyperlink{eqloss}{{[}eqloss{]}}, the policy gradient method
uses the following gradient:

\[\begin{aligned}
\nabla_\theta L(\theta) &= - \mathbb{E}_{\tau \sim \pi(\tau | \theta)} [\Psi \nabla_\theta \text{log} \pi(\cdot | \theta)]**** 
\end{aligned}\]

where \(\Psi\) is typically chosen as an advantage function, \(A\),
which has the general form of: \(A(a_t, s_t) = r(\tau)_t - V(s_t)\),
where \(V(s_t)\) is the expected cumulative reward of the policy in
state \(s_t\). In our experiments, we set \(\Psi\) to use the
generalized advantage estimation method (GAE) {[}@gae{]} which involves
training a critic network to estimate \(V(s_t)\). While the policy
gradient method directly optimizes
\protect\hyperlink{pgrad}{{[}pgrad{]}}, doing so often results in
high-variance gradient estimates which leads to unstable training and
poor performance {[}@mohamed2020monte{]}.

\hypertarget{natural-policy-gradient-methods}{%
\subsection{Natural Policy Gradient
Methods}\label{natural-policy-gradient-methods}}

To stabilize training, the natural policy gradient method
{[}@Amari1998{]} restricts how much the policy can change across
training iterations by adding a Kullback--Leibler divergence constraint
(\(D_{KL}\)) between policy iterations:

\[\theta^{(k+1)} = \underset{\theta^{(k+1)}}{\mathop{\mathrm{argmin}}} \, L(\theta^{(k+1)}) + \lambda D_{KL}(\pi(\cdot | \theta^{(k)}), \pi(\cdot | \theta^{(k+1)})) ****\]

where \(\theta^{(k)}\) defines the parameters at optimization iteration
\(k\). To approximately solve
\protect\hyperlink{ngrad_deriv}{{[}ngrad\_deriv{]}}, we use a
first-order taylor-series approximation of \(L\) around
\(\theta^{(k)}\), a second-order taylor-series approximation of
\(D_{KL}\), and solve for the optimum (see {[}@natural\_lec{]} and
{[}@natural\_grad\_blog{]} for a full derivation). Doing so, we derive
the natural policy gradient method,

\[\theta^{(k+1)} = \theta^{(k)} - {\lambda}^{-1} {F}^{-1} \nabla L(\theta^{(k)})
    ****\]

where \(F\) is the Fisher-information matrix:

\[F = \mathbb{E}_{\pi(\cdot |\theta)} [\nabla_\theta \log \pi(\cdot |\theta) \nabla_\theta \log \pi(\cdot |\theta)^T]\]

\begin{figure}
\centering
\includegraphics{strats.pdf}
\caption{image}
\end{figure}

\hypertarget{approximations-and-related-work}{%
\section{Approximations and Related
Work}\label{approximations-and-related-work}}

A key problem is that the Fisher-information matrix (\(F\)) is an
\(n_\theta \times n_\theta\) matrix, where \(n_\theta\) is the number of
parameters in the model. For neural networks which can have tens of
millions of parameters, directly computing the inverse of the
Fisher-information matrix is intractable. This has led to rising
interest by the research community to develop new ways to approximate
the inverse of the Fisher-information matrix for neural networks.
However, most of these approximations have only been investigated in
computer vision tasks and not in reinforcement learning (RL) tasks.
Below, we review some of the most popular approximations and their
related work in RL.

\textbf{Diagonal Approximations (Diagonal)} {[}@diagonal{]}: Diagonal
approximations use a diagonal approximation of \(F\). This makes storage
and inversion easy, however, it ignores a large amount of curvature
information. While some RL research {[}@gu2017qprop{]} indirectly use
the diagonal approximation by using the Adam optimizer
{[}@kingma2017adam{]}, there has not been any specific focus on
understanding the fundamental trade-offs when using Diagonal
approximations compared to other approximations when realizing the
natural policy gradient.

\textbf{Hessian-free Approximations (HF)} {[}@hessianfree{]}:
Hessian-free approximations use matrix-vector products and the conjugate
gradient method to approximately solve for
\({F}^{-1} \nabla L(\theta)\). However, computing the conjugate gradient
at each iteration can be computationally expensive. One of the most
popular implementations of the natural policy gradient which used the HF
approximation is Trust region policy optimization (TRPO) {[}@trpo{]}
which used a backtracking line search method to achieve state-of-the-art
results in continuous control tasks at the time.

\textbf{Kronecker-factor Approximations (KFAC/EKFAC)} {[}@kfac{]}:
Kronecker-factor approximations use a block-diagonal approximation of
\(F\) which assumes each layer is independent of the others. KFAC
{[}@kfac{]} decomposes the Fisher-information matrix using the Kronecker
product. EKFAC {[}@ekfac{]} uses a different approximation based on KFAC
which showed improved results across computer vision experiments. In RL,
Actor-critic using kronecker-factored trust region (ACKTR) {[}@acktr{]}
used KFAC optimization and step-size clipping to realize the natural
policy gradient and showed improved results compared to TRPO. EKFAC has
not been investigated in the RL literature.

\textbf{Woodbury Approximations (TENGraD)} {[}@tengrad{]}: While EKFAC
proposes an improved approximation to KFAC, TENGraD provides an exact
block-diagonal approximation using the Woodbury identity. However,
TENGraD requires constructing a \(m \times m\) matrix where \(m\) is the
batch size which can be computationally expensive when using large batch
sizes. TENGraD has not been investigated in the RL literature.

\hypertarget{training-strategies}{%
\section{Training Strategies}\label{training-strategies}}

In this section, we introduce the collection of strategies that we will
conduct a deep exploration into to improve the performance of natural
policy gradient methods. The proposed collection of strategies can be
applied universally to significantly improve performance for all
second-order approximations and is particularly effective when combined.
Figure \protect\hyperlink{fig:strats}{{[}fig:strats{]}} shows a diagram
of the two training strategies.

\hypertarget{batch-size-tuning}{%
\subsection{Batch Size Tuning}\label{batch-size-tuning}}

In the policy gradient setting, the batch size defines how many training
examples to collect in the environment before using the collected data
to update the model. Using a larger batch size will result in more
examples, for a more stable update, but fewer model updates per
environment step. Comparatively, using a smaller batch size will result
in fewer examples, for a less stable update, but more updates per
environment step. Although the importance of the batch size is not
emphasized much in the literature, we find that tuning the batch size is
a critical training strategy that can significantly affect the final
performance and other metrics of the model (a similar result was found
for Q-learning methods {[}@Kielak2020{]}). To understand how a tuned
batch size can improve the baseline performance, we tune the batch size
of the baseline models based on the performance metric, re-conduct the
training across all environments, and compare the change in metrics to
the baseline. For succinctness, we show the results of batch size tuning
in Appendix \protect\hyperlink{sec:batch_results}{7} and show the
results of applying both training strategies in Section
\protect\hyperlink{sec:training_strats}{5.2}.

\begin{figure}
\centering
\includegraphics{performance.pdf}
\caption{image}
\end{figure}

\begin{longtable}[]{@{}lrrrr@{}}
\toprule()
Approximation & Performance & Stability & Sample Efficiency &
Computation Time \\
\midrule()
\endhead
Diagonal & 12.52 & -12338.0 & -2170.0 & \textbf{-37.051} \\
HF & 68.73 & \textbf{-107.0} & -1708.0 & -37.282 \\
KFAC & 29.03 & -178.0 & \textbf{-1263.0} & -37.430 \\
EKFAC & 61.85 & -235.0 & -1316.0 & -37.624 \\
TENGraD & \textbf{85.69} & -182.0 & -1425.0 & -52.861 \\
\bottomrule()
\end{longtable}

\hypertarget{natural-critic-optimization}{%
\subsection{Natural Critic
Optimization}\label{natural-critic-optimization}}

Another training strategy is to improve the optimization of the critic
network. A standard approach is to optimize the critic using SGD;
however, this can sometimes lead to unstable model updates which
negatively affect the final performance. Some other work investigated
using clipped targets to stabilize training
{[}@engstrom2020implementation{]}. Later, ACKTR {[}@acktr{]} used the
natural gradient to further improve the stability and showed improved
performance using KFAC optimization for both the policy and the critic
network. More specifically, while ACKTR investigated applying only KFAC
optimization to both the policy network and the critic network, we
investigate five different second-order approximations for the policy
network and for each of these we investigate five second-order
approximations for tuning the critic network. Furthermore, we explore
how optimizing the critic network with the natural gradient affects four
key metrics. To achieve this, we leverage the models with a tuned batch
size and through grid search, find the best approximation to optimize
the critic network, re-conduct the training across all environments, and
compare the change in metrics to the baseline. The results are shown in
Section \protect\hyperlink{sec:training_strats}{5.2}.

\hypertarget{experiments}{%
\section{Experiments}\label{experiments}}

In this section, we investigate the performance of the five second-order
approximations and the effect of our training strategies. Furthermore,
in doing so, we also investigate the performance of EKFAC and TENGraD
approximations for natural policy gradient reinforcement learning for
the first time in the literature. We compare each approximation across
seven different MuJoCo environments: HalfCheetah-v2, Ant-v2, Hopper-v2,
Humanoid-v2, Walker2d-v2, Reacher-v2, and Swimmer-v2. All experiments
were run across 10 different random seeds.

Throughout the experiments, we study four metrics: \textbf{Performance}
which is the maximum average return achieved by the policy across
training; \textbf{Stability} which is the average standard deviation
(across seeds) across training; \textbf{Sample Efficiency} which is the
number of environment steps to achieve a specific performance threshold;
and \textbf{Computation Time} which is the amount of time to take 100K
environment steps while training. More information on these metrics is
available in Appendix \protect\hyperlink{sec:metrics}{8}.

For clarity purposes, to make all metrics correspond with `larger is
better', we flip the sign of the metrics where smaller values are better
(i.e., Stability, Sample Efficiency, and Computation Time). For example,
if two agents achieve an average standard deviation (across seeds) of
500 and 600 (where 500 is a smaller standard deviation and is thus more
stable), we flip the signs to get -500 and -600, in which case the
policy with the larger value of -500 is more stable and is therefore
considered better. All hyperparameter information can be found in
Appendix \protect\hyperlink{sec:hparams}{9}.

\hypertarget{baseline}{%
\subsection{Baseline}\label{baseline}}

\begin{figure}
\centering
\includegraphics{metrics.pdf}
\caption{image}
\end{figure}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 1687 (+67\%) & -439 (+16\%) & -2775 (-50\%) & -22
(+18\%) \\
Ant-v2 & \textbf{825 (+94\%)} & \textbf{-178 (+100\%)} & \textbf{-1025
(+10\%)} & -43 (+18\%) \\
Hopper-v2 & 527 (-55\%) & -48 (+87\%) & NaN & -27 (+16\%) \\
Humanoid-v2 & 486 (-33\%) & -20 (+72\%) & NaN & \textbf{-50 (+19\%)} \\
Walker2d-v2 & 526 (-71\%) & -59 (+83\%) & -2175 (-222\%) & -28
(+18\%) \\
Reacher-v2 & -12 (+14\%) & -304 (+92\%) & -625 (-34\%) & \textbf{-21
(+19\%)} \\
Swimmer-v2 & 33 (-10\%) & -4 (+7\%) & NaN & -22 (+15\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 1506 (+32\%) & -216 (-423\%) & \textbf{-1120 (+62\%)} &
-29 (-6\%) \\
Ant-v2 & \textbf{1573 (+65\%)} & -143 (-189\%) & -1370 (+57\%) & -54
(-3\%) \\
Hopper-v2 & 504 (-78\%) & -45 (+85\%) & NaN & -34 (-3\%) \\
Humanoid-v2 & 499 (-39\%) & -13 (+60\%) & NaN & -62 (-3\%) \\
Walker2d-v2 & 398 (-86\%) & \textbf{-35 (+89\%)} & NaN & -36 (-4\%) \\
Reacher-v2 & -4 (+11\%) & -0 (+63\%) & -270 (+44\%) & -29 (-9\%) \\
Swimmer-v2 & 47 (+15\%) & -5 (-57\%) & -820 (+35\%) & -30 (-12\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 2319 (+38\%) & -396 (-52\%) & -480 (+29\%) & -27
(-1\%) \\
Ant-v2 & \textbf{2593 (+65\%)} & -386 (-106\%) & -240 (+38\%) & -52
(+0\%) \\
Hopper-v2 & 494 (-60\%) & \textbf{-86 (+85\%)} & NaN & \textbf{-32
(+2\%)} \\
Humanoid-v2 & 451 (-36\%) & -34 (+48\%) & NaN & -62 (-0\%) \\
Walker2d-v2 & 337 (-24\%) & -95 (+36\%) & NaN & -35 (+1\%) \\
Reacher-v2 & -7 (+19\%) & -1 (-40\%) & -360 (-14\%) & -26 (+1\%) \\
Swimmer-v2 & 52 (+53\%) & -15 (-87\%) & \textbf{-1770 (+53\%)} & -27
(+1\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 2513 (+11\%) & -603 (-17\%) & -570 (+0\%) & -27
(-1\%) \\
Ant-v2 & \textbf{2345 (+50\%)} & -325 (-10\%) & \textbf{-375 (+38\%)} &
-52 (-0\%) \\
Hopper-v2 & 495 (-74\%) & \textbf{-66 (+86\%)} & NaN & \textbf{-33
(+4\%)} \\
Humanoid-v2 & 456 (-37\%) & -21 (+35\%) & NaN & -63 (-0\%) \\
Walker2d-v2 & 403 (-72\%) & -72 (+77\%) & NaN & -36 (-2\%) \\
Reacher-v2 & -6 (+10\%) & -1 (+36\%) & -615 (-5\%) & -27 (-2\%) \\
Swimmer-v2 & 37 (-11\%) & -7 (+12\%) & -2910 (-169\%) & -27 (-1\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 2058 (+15\%) & -592 (-69\%) & -788 (+52\%) & -44
(-5\%) \\
Ant-v2 & 3855 (+113\%) & -464 (-153\%) & -652 (+59\%) & -71 (-4\%) \\
Hopper-v2 & 1510 (-14\%) & -148 (+35\%) & -4256 (-1008\%) & -50
(-4\%) \\
Humanoid-v2 & 640 (-26\%) & \textbf{-21 (+60\%)} & NaN & -79 (-2\%) \\
Walker2d-v2 & 1614 (-41\%) & -267 (+41\%) & -1296 (-89\%) & -53
(-4\%) \\
Reacher-v2 & -5 (+13\%) & -1 (-16\%) & -208 (+43\%) & -43 (-4\%) \\
Swimmer-v2 & \textbf{130 (+181\%)} & -49 (-874\%) & \textbf{-172
(+86\%)} & -44 (-4\%) \\
\bottomrule()
\end{longtable}

We first investigate each approximation's baseline performance using the
same batch size and using SGD to optimize the critic network. The
training curves of the different approximations are shown in Figure
\protect\hyperlink{fig:baseline}{{[}fig:baseline{]}}. The solid-colored
line represents the mean value across the random seeds and the shaded
region represents one standard deviation above and below the mean. We
also show the mean metrics across the seven different environments in
Table \protect\hyperlink{tab:baseline}{{[}tab:baseline{]}}.

\textbf{Performance} Since each environment has different reward scales,
to weigh each environment's score equally, we normalize the performance
scores in Table \protect\hyperlink{tab:baseline}{{[}tab:baseline{]}} and
Figure
\protect\hyperlink{fig:metrics_baseline}{{[}fig:metrics\_baseline{]}}.

Figure \protect\hyperlink{fig:baseline}{{[}fig:baseline{]}} shows that
no approximation outperforms all other approximations across all
environments and shows that the best approximation depends on the
environment. Table \protect\hyperlink{tab:baseline}{{[}tab:baseline{]}}
shows TENGraD achieves the best performance score across all
approximations, followed by HF and EKFAC, followed by KFAC and lastly
Diagonal. Table \protect\hyperlink{tab:baseline}{{[}tab:baseline{]}}
also shows that improved approximations can lead to improved performance
since TENGraD achieves the best mean performance score across all
environments and is the most accurate approximation. We also see that
the Diagonal achieves the lowest performance score and that in some
environments (Ant-v2 and Reacher-v2 shown in Figure
\protect\hyperlink{fig:baseline}{{[}fig:baseline{]}}) it diverges near
the end of the training; likely because it ignores a large amount of
curvature leading to unstable updates.

Figure
\protect\hyperlink{fig:metrics_baseline}{{[}fig:metrics\_baseline{]}}
shows normalized performance scores across four aggregate metrics with
95\% stratified bootstrap confidence intervals from
{[}@agarwal2021deep{]} including median, interquartile mean (IQM), mean,
and the optimality gap across all approximations. A larger score in the
median, IQM, and mean aggregations and a smaller score in the optimality
gap aggregation corresponds to better performance.

We see TENGraD significantly outperforms the other approximations in
terms of the IQM, mean, and optimality gap aggregation metrics because
it achieves the best score and there is no overlap between its
confidence intervals and the others. EKFAC and HF achieve the
second-best scores however, their confidence intervals overlap which
shows their performance is not significantly different from each other.
Lastly, we see KFAC achieves the third-best score, followed by Diagonal
with the worst score. Analyzing the median metrics in Figure
\protect\hyperlink{fig:metrics_baseline}{{[}fig:metrics\_baseline{]}} is
not as straightforward due to a large amount of overlap in confidence
intervals; this is not surprising since the median is a poor measure of
overall performance {[}@agarwal2021deep{]}. We see TENGraD is
significantly better than all other approximations other than EKFAC; and
that EKFAC is significantly better than Diagonal. Interestingly, the
median aggregate metric shows a trend that newer second-order
approximations lead to better median performance.

\textbf{Stability} HF achieves the best stability score, closely
followed by KFAC, followed by TENGraD and EKFAC, and lastly, with a
significantly lower score, Diagonal. HF achieves the best stability
score, likely because it utilizes the conjugate gradient algorithm for
its update. Whereas Diagonal achieves the lowest score, likely because
its approximation ignores a large amount of curvature leading to
inaccurate gradient scaling. We see in the HalfCheetah-v2 and Reacher-v2
environments, Diagonal is unable to remain stable throughout training
and diverges at the end of training.

\textbf{Sample Efficiency} KFAC achieves the best sample efficiency
score, closely followed by EKFAC and TENGraD, followed by HF and
Diagonal.

\textbf{Computation Time} Diagonal achieves the best computation time
score, followed by HF, followed by KFAC and EKFAC, and lastly TENGraD.
Diagonal achieves the best scores due to its simple and efficient
implementation, only requiring an element-wise multiplication and
division. Whereas, TENGraD achieves the lowest score due to it having to
periodically compute the inverse of a very large \(m \times m\) matrix
where \(m\) is the batch size.

\hypertarget{sec:training_strats}{%
\subsection{Training Strategies}\label{sec:training_strats}}

We now investigate how we can leverage a performance-tuned batch size
and use the natural gradient to optimize the critic network to achieve
performance improvements across all approximations in Tables
\protect\hyperlink{tab:diagonal_tuned}{{[}tab:diagonal\_tuned{]}} -
\protect\hyperlink{tab:tengrad_tuned}{{[}tab:tengrad\_tuned{]}}. In all
the tables we show the percentage change compared to the baseline model
in brackets and bold the largest improvement for each metric. If the
policy is unable to achieve the sample efficiency threshold compared to
the baseline we show `NaN'.

\textbf{Key Trends:} Overall, we see tuning the batch size and using the
natural gradient to optimize the critic network can lead to significant
improvements in performance, training stability, sample efficiency, and
speed in many reinforcement learning environments across all five
natural gradient approximations. Specifically, we see TENGraD achieves
improvements in performance, stability, and sample efficiency of up to
+181\%, +60\%, and +86\% respectively with at most a 5\% decrease in the
speed score. The results of applying the strategies across all the other
approximations are summarized in their respective table captions.

Interestingly, we see that using the training strategies the metrics are
usually improved in the HalfCheetah-v2, Ant-v2, Reacher-v2, and
Swimmer-v2 environments, however, the other environments such as
Hopper-v2, Humanoid-v2, and Walker2d-v2 see results decrease compared to
the baseline. This may be because the strategies are tuned on the
HalfCheetah-v2 environment which is much similar to the environments in
which the policy performed well in and is not similar to the
environments in which the policy performed poorly. We hypothesis that
tuning the strategies on the poor performance environments can result in
similar performance improvements seen in the other environments. We
leave this for future research.

Another trend we see is that when the performance score is improved
usually the stability score decreases; and when the performance score is
improved, we see a similar improvement in the sample efficiency score.

\hypertarget{conclusion}{%
\section{Conclusion}\label{conclusion}}

In this paper, we systematically examined how tuning the batch size and
optimizing the critic network with the natural gradient can be effective
training strategies to yield significant performance improvements for
the natural policy gradient method; and that these strategies are
effective across all five different approximations. Furthermore, we
investigated how optimizing for performance affects other metrics such
as training stability, sample efficiency, and computational time. We
found using the proposed collection of training strategies can achieve
performance and sample efficiency improvements ranging up to +181\% and
+86\% respectively across the MuJoCo control benchmark and that TENGraD
achieved the best performance out of all the approximations. We also
find that there is a fundamental trade-off between achieving high
performance and maintaining stability throughout training, and that
performance is positively correlated with sample efficiency. We hope
this research helps expand our field's understanding of how different
approximations and training strategies affects the natural policy
gradient and helps practitioners efficiently leverage natural policy
gradient methods for real-world reinforcement learning tasks.

\hypertarget{sec:batch_results}{%
\section{Tuned Batch Size Results}\label{sec:batch_results}}

We show the results of tuning the batch size across all approximations
in Tables
\protect\hyperlink{tab:diag_batch_tuned}{{[}tab:diag\_batch\_tuned{]}} -
\protect\hyperlink{tab:tengrad_batch_tuned}{{[}tab:tengrad\_batch\_tuned{]}}.
We found KFAC's tuned batch size was the same as its baseline batch size
so we don't include its results. We see large improvements in
performance, stability, sample efficiency, and speed across all
approximations showing that tuning the batch size is a key strategy for
achieving the best performance.

\hypertarget{sec:metrics}{%
\section{More Details on the Metrics}\label{sec:metrics}}

For the sample efficiency metric, the performance thresholds are
computed for each environment as the lowest performance score across all
approximations in the baseline experiments. The thresholds are then held
constant throughout the rest of the experiments. For clarity purposes,
the threshold scores are divided by 1000. The exact thresholds used are
made available in our code repository.

In Table \protect\hyperlink{tab:baseline}{{[}tab:baseline{]}}, since
each environment has different reward scales, to weigh each
environment's score equally, we normalize the performance scores of each
environment by dividing by the highest score achieved in that
environment across all approximations and multiplying it by 100, making
the largest achievable reward 100. We don't scale the values by 100 for
Figure
\protect\hyperlink{fig:metrics_baseline}{{[}fig:metrics\_baseline{]}}.

\hypertarget{sec:hparams}{%
\section{Hyperparameters}\label{sec:hparams}}

\hypertarget{baseline-1}{%
\subsection{Baseline}\label{baseline-1}}

For the baseline model, we tuned the following hyperparameters for one
million environment steps: damping parameter with values (1e-1 1e-2),
critic learning rate with values (1e-2 1e-3), whether to use a
backtracking line search or not based on {[}@trpo{]}, when not using
line search we use step-size clipping used in {[}@acktr{]} and tune the
maximum learning rate with values (1e-1 1e-2). All approximations used a
batch size of 15K except for TENGraD which used a batch size of 6K
because our GPUs didn't have enough memory for a batch size of 15K. We
chose 15K because it is commonly used in the literature {[}@trpo;
@acktr{]}.

Although TENGraD uses a smaller batch size which may be seen as unfair
due to the increased number of optimization steps, comparing all
approximations with their tuned batch sizes (with available batch sizes
smaller than TENGraD's batch sizes), TENGraD still achieves the highest
performance score.

All hyperparameters used in all the experiments can be found in our code
repository.

\hypertarget{batch-size-tuning-1}{%
\subsection{Batch Size Tuning}\label{batch-size-tuning-1}}

For the batch size model, we tuned the batch size for five million
environment steps with values (25 20 15 10 5) except for TENGraD,
because of limited GPU memory, which we searched over values (10 8 6 4).
EKFAC's performance on HalfCheetah-v2 (which it was tuned on) decreased
with the tuned batch size so we used the baseline batch size when
applying the natural critic optimization.

\hypertarget{natural-critic-optimization-1}{%
\subsection{Natural Critic
Optimization}\label{natural-critic-optimization-1}}

For the natural critic optimization model, we applied a grid search over
the following hyperparameters for five million environment steps:
natural gradient approximation with values (Diagonal HF KFAC EKFAC
TENGraD), critic damping parameter with values (1e-1 1e-2), whether to
use a backtracking line search or not based on {[}@trpo{]}, when not
using line search we use step-size clipping used in {[}@acktr{]} and
tune the maximum learning rate with values (1e-1 1e-2).

\hypertarget{model-architectures}{%
\section{Model Architectures}\label{model-architectures}}

The policy and critic models consisted of three linear layers with 64
hidden units each using the tanh activation function, except for the
final output. Following standard practice, all layers were initialized
with orthogonal initialization.

\hypertarget{code}{%
\section{Code}\label{code}}

For fisher approximation implementations we implemented the diagonal
ourselves; we used {[}@pytroch\_trpo{]} as a reference when implementing
HF; we used the code provided by EKFAC {[}@ekfac{]} for EKFAC and KFAC;
and we used the authors provided code for the implementation of TENGraD.

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 1371 (+36\%) & -257 (+51\%) & -2250 (-22\%) & -22
(+18\%) \\
Ant-v2 & \textbf{668 (+57\%)} & \textbf{-100 (+100\%)} & -1575 (-38\%) &
-43 (+17\%) \\
Hopper-v2 & 1500 (+29\%) & -330 (+10\%) & \textbf{-1125 (+5\%)} & -27
(+17\%) \\
Humanoid-v2 & 749 (+3\%) & -42 (+42\%) & -4775 (-9\%) & \textbf{-50
(+19\%)} \\
Walker2d-v2 & 1802 (+0\%) & -210 (+40\%) & -1275 (-89\%) & -28
(+18\%) \\
Reacher-v2 & -12 (+8\%) & -1912 (+48\%) & -775 (-67\%) & -21 (+18\%) \\
Swimmer-v2 & 36 (-2\%) & -4 (+18\%) & -4025 (-19\%) & -22 (+18\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 1338 (+17\%) & -171 (-314\%) & \textbf{-1900 (+35\%)} &
-28 (-5\%) \\
Ant-v2 & 1123 (+18\%) & -92 (-85\%) & -2630 (+17\%) & -54 (-3\%) \\
Hopper-v2 & 2358 (+3\%) & -340 (-14\%) & -510 (+17\%) & -35 (-4\%) \\
Humanoid-v2 & \textbf{991 (+21\%)} & -47 (-42\%) & -3680 (+16\%) & -63
(-3\%) \\
Walker2d-v2 & 3065 (+8\%) & -298 (+7\%) & -690 (+6\%) & -37 (-5\%) \\
Reacher-v2 & -5 (+1\%) & \textbf{-0 (+24\%)} & -360 (+25\%) & -28
(-7\%) \\
Swimmer-v2 & 41 (-1\%) & -5 (-49\%) & -1200 (+5\%) & -29 (-10\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 2200 (-3\%) & -460 (+11\%) & -430 (+25\%) & -28
(-5\%) \\
Ant-v2 & \textbf{1725 (+10\%)} & -346 (-18\%) & -400 (+33\%) & -54
(-4\%) \\
Hopper-v2 & 1097 (-43\%) & -457 (+5\%) & NaN & \textbf{-34 (+4\%)} \\
Humanoid-v2 & 788 (+8\%) & -80 (-148\%) & -3940 (+17\%) & -65 (-4\%) \\
Walker2d-v2 & 1337 (-7\%) & -519 (-66\%) & -400 (+33\%) & -36 (-3\%) \\
Reacher-v2 & -8 (-14\%) & \textbf{-1 (+17\%)} & \textbf{-370 (+37\%)} &
-27 (-4\%) \\
Swimmer-v2 & 41 (-1\%) & -7 (+1\%) & -2430 (-125\%) & -29 (-8\%) \\
\bottomrule()
\end{longtable}

\begin{longtable}[]{@{}lllll@{}}
\toprule()
Environment & Performance & Stability & Sample Efficiency & Speed \\
\midrule()
\endhead
HalfCheetah-v2 & 1943 (+8\%) & -371 (-6\%) & -1220 (+25\%) & -42
(-1\%) \\
Ant-v2 & 1998 (+10\%) & -236 (-28\%) & -1356 (+14\%) & -69 (-1\%) \\
Hopper-v2 & 1870 (+7\%) & -318 (-40\%) & -340 (+11\%) & -49 (-1\%) \\
Humanoid-v2 & \textbf{972 (+13\%)} & \textbf{-49 (+6\%)} & -3728 (+11\%)
& -79 (-2\%) \\
Walker2d-v2 & 2788 (+2\%) & -576 (-27\%) & -496 (+27\%) & -51 (-0\%) \\
Reacher-v2 & -6 (-14\%) & -1 (-63\%) & -268 (+27\%) & -42 (-0\%) \\
Swimmer-v2 & 45 (-3\%) & -6 (-24\%) & \textbf{-452 (+64\%)} & -43
(-1\%) \\
\bottomrule()
\end{longtable}

